Data Splits and Metrics for Method Benchmarking on Surgical Action Triplet Datasets

In addition to generating data and annotations, devising sensible data splitting strategies and evaluation metrics is essential for the creation of a benchmark dataset. This practice ensures consensus on the usage of the data, homogeneous assessment, and uniform comparison of research methods on the dataset. This study focuses on CholecT50, which is a 50 video surgical dataset that formalizes surgical activities as triplets of <instrument, verb, target>. In this paper, we introduce the standard splits for the CholecT50 and CholecT45 datasets and show how they compare with existing use of the dataset. CholecT45 is the first public release of 45 videos of CholecT50 dataset. We also develop a metrics library, ivtmetrics, for model evaluation on surgical triplets. Furthermore, we conduct a benchmark study by reproducing baseline methods in the most predominantly used deep learning frameworks (PyTorch and TensorFlow) to evaluate them using the proposed data splits and metrics and release them publicly to support future research. The proposed data splits and evaluation metrics will enable global tracking of research progress on the dataset and facilitate optimal model selection for further deployment.

==> table/c2c.tex <==
\begin{table}[htp]
\centering
    \setlength{\tabcolsep}{5pt}
    \captionsetup{skip=0pt,singlelinecheck=off,justification=raggedright}
    \caption{Cholec80 to CholecT45 video filename mapping.}
    \label{table:c2c}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{@{}llrllrll@{}}
        \toprule
        Cholec80  & CholecT45 & \phantom{abc} & Cholec80  & CholecT45 &\phantom{abc} & Cholec80  & CholecT45 \\ 
        \midrule
        7013HD Bin.01-H264-480 & VID01 && 8425HD Bin.01-H264-480 & VID26 && 9066HD Bin.01-H264-480 & VID52 \\ 
        7201HD Bin.01-H264-480 & VID02 && 8554HD Bin.02-H264-480 & VID27 && 9245HD Bin.01-H264-480 & VID56 \\ 
        7301HD Bin.01-H264-480 & VID04 && 8577HD Bin.01-H264-480 & VID29 && 9285HD Bin.01-H264-480 & VID57 \\ 
        7345HD-H264-480	& VID05 && 8611HD Bin.01-H264-480 & VID31 && 9361HD Bin.01-H264-480 & VID60 \\ 
        7348HD Bin.01-H264-480 & VID06 && 8667HD Bin.01-H264-480 & VID32 && 9443HD Bin.01-H264-480 & VID62 \\ 
        7487HD Bin.01-H264-480 & VID08 && 8897HD Bin.01-H264-480 & VID35 && 9544HD Bin.01-H264-480 & VID65 \\ 
        7535HD Bin.01-H264-480 & VID10 && 8906HD Bin.01-H264-480 & VID36 && 9559HD Bin.01-H264-480 & VID66 \\ 
        7695HD Bin.01-H264-480 & VID12 && 9292HD Bin.01-H264-480 & VID40 && 9624HD Bin.01-H264-480 & VID68 \\ 
        7697HD Bin.01-H264-480 & VID13 && 7699HD Bin.01-H264-480 & VID42 && 9674HD Bin.01-H264-480 & VID70 \\ 
        7719HD Bin.01-H264-480 & VID14 && 7947HD Bin.01-H264-480 & VID43 && 9764HD Bin.01-H264-480 & VID73 \\ 
        7754HD Bin.01-H264-480 & VID15 && 8353HD Bin.01-H264-480 & VID47 && 9955HD Bin.01-H264-480 & VID74 \\ 
        7964HD Bin.01-H264-480 & VID18 && 8714HD Bin.01-H264-480 & VID48 && 9966HD Bin.01-H264-480 & VID75 \\ 
        8123HD Bin.01-H264-480 & VID22 && 8823HD Bin.01-H264-480 & VID49 && 10133HD Bin.01-H264-1080 & VID78 \\ 
        8132HD-H264-480 & VID23 && 8852HD Bin.01-H264-480 & VID50 && 10206HD Bin.01-H264-1080	& VID79 \\ 
        8307HD Bin.01-H264-480 & VID25 && 8870HD Bin.01-H264-480 & VID51 && 10241HD Bin.01-H264-1080 & VID80 \\
        \bottomrule
        \end{tabular}
    }
\end{table}
